DLPaper2Code: Auto-generation of Code from Deep Learning Research Papers

With an abundance of research papers in deep learning, reproducibility or adoption of the existing works becomes a challenge. This is due to the lack of open source implementations provided by the authors. Further, re-implementing research papers in a different library is a daunting task. To address these challenges, we propose a novel extensible approach, DLPaper2Code, to extract and understand deep learning design flow diagrams and tables available in a research paper and convert them to an abstract computational graph. The extracted computational graph is then converted into execution ready source code in both Keras and Caffe, in real-time. An arXiv-like website is created where the automatically generated designs is made publicly available for 5,000 research papers. The generated designs could be rated and edited using an intuitive drag-and-drop UI framework in a crowdsourced manner. To evaluate our approach, we create a simulated dataset with over 216,000 valid design visualizations using a manually defined grammar. Experiments on the simulated dataset show that the proposed framework provide more than $93\%$ accuracy in flow diagram content extraction.

==> 2_Literature.tex <==
\section{Literature Study}

The umbrella of extracting and analyzing figures and charts from scholarly publications are studied in literature~\cite{choudhury2015architecture, ray2015automatic}. B{\"o}schen and Scherp~\cite{boschen2015formalization} proposed a pipeline for extracting textual information from infographics. Lee et al.~\cite{lee2017viziometrics} created \textit{Viziometrics}, a tool for analyzing and inferring information from visual content in a scholarly publication. Chen et al.~\cite{chen2015diagramflyer} design a query system to search content over bar charts and scatter plots in pdf documents. Al-Zaidy and Giles~\cite{al2017machine} extracted richer metadata from 2D plots in a scholarly paper for better semantic indexing of document and search retrieval. However, to the best of our knowledge, there is no directly related work to extract flow diagram information about deep learning models from research papers and convert them into execution ready source code.

In the paper PDFFigures2.0~\cite{clark2016pdffigures} the authors present a rule mining based approach for analyzing the structure of a document.They do this by detecting captions, graphical elements and chunks of body text.This procedure produces a rich decomposition of the document and analysis of the text.They achieve 94\% precision at 90\%recall on newly contributed CS150 dataset by the authors in the same paper. Chowdhury et al. in the paper Figure metadata extraction from Digital Documents~\cite{choudhury2013figure} describe an extraction process which is able to extract captions and mentions relating to a figure.This extraction process has three distinct steps : Extraction of figures and text, Extraction of Captions and Matching of Captions with figures.For the purpose of extracting captions the authors give a rule mining based system and a Machine Learning based system wherein they train Naive Bayes classifier and Support vector machine for determination of caption and non caption sentences in the text.

The paper Summarizing Figures , Tables and Algorithms in Scientific Papers to Augment Search Results~\cite{bhatia2012summarizing} by Bhatia et al. gives a process for generating the synopsis of document elements like Figures and tables.The authors note the fact that only the caption is not capable of explaning the document element.The method proposed here involves preprocessing of the document by extracting the text, caption parsing, sentence segmentation and reference sentence parsing.Preprocessing is followed by feature extraction based on content based features and context based features.The extracted features are classified using Naive Bayes and Support Vector Machines.Finally a utility function is defined which determines which sentences are to be included in the synopsis of a document element.
 



